Towards Visual Taxonomy Expansion

Taxonomy expansion task is essential in organizing the ever-increasing volume of new concepts into existing taxonomies. Most existing methods focus exclusively on using textual semantics, leading to an inability to generalize to unseen terms and the "Prototypical Hypernym Problem." In this paper, we propose Visual Taxonomy Expansion (VTE), introducing visual features into the taxonomy expansion task. We propose a textual hypernymy learning task and a visual prototype learning task to cluster textual and visual semantics. In addition to the tasks on respective modalities, we introduce a hyper-proto constraint that integrates textual and visual semantics to produce fine-grained visual semantics. Our method is evaluated on two datasets, where we obtain compelling results. Specifically, on the Chinese taxonomy dataset, our method significantly improves accuracy by 8.75 %. Additionally, our approach performs better than ChatGPT on the Chinese taxonomy dataset.

==> paper/8-limitations.tex <==
\clearpage
\section*{Limitations}
In this section, we will discuss the potential limitations of our framework.
The major limitation is that not all concepts have corresponding images, especially some abstract concepts. These images of abstract concepts cannot provide additional semantics for terms.
For example, terms like \texttt{Idealism} and words like \texttt{Hello} have no image to depict the definition or present its properties. They are created and defined by humans, lacking the corresponding instances in real life. In cases like these, term definitions are more helpful in enriching their semantics.

\section*{Ethical Considerations}
There are two main ethical considerations:
1) Since our Chinese hypernymy dataset is sourced from user behaviors on the Meituan platform, there may be an ethical issue with harmful content (e.g., personal privacy information, racist language, violent images, and pornographic images). After our analysis and manual testing, our dataset is free of this ethical issue for two reasons. First, Meituan has its content filter, which has been reviewed by the Meituan ethics review board, to remove dirty content automatically. We eliminate all user-related information from sources. Second, we randomly select 3,000 images from the dataset and assign them to the annotators for manual evaluation. The results show no harmful images or personal information leakage in the testing samples.
2) Since our hypernymy pairs and images are from Meituan, we need to follow the copyright of Meituan. Protocols agreed upon by Meituan users allow us to use anonymous user data for research purposes and distribution for non-commercial purposes. The hypernymy pairs and images in our dataset are distributed under Creative Commons Non-Commercial (CC-NC) license, where the NC component prohibits anyone from using our constructed dataset for commercial purposes.
